Deep Flow-Guided Video Inpainting

Video inpainting, which aims at filling in missing regions of a video, remains challenging due to the difficulty of preserving the precise spatial and temporal coherence of video contents. In this work we propose a novel flow-guided video inpainting approach. Rather than filling in the RGB pixels of each frame directly, we consider video inpainting as a pixel propagation problem. We first synthesize a spatially and temporally coherent optical flow field across video frames using a newly designed Deep Flow Completion network. Then the synthesized flow field is used to guide the propagation of pixels to fill up the missing regions in the video. Specifically, the Deep Flow Completion network follows a coarse-to-fine refinement to complete the flow fields, while their quality is further improved by hard flow example mining. Following the guide of the completed flow, the missing video regions can be filled up precisely. Our method is evaluated on DAVIS and YouTube-VOS datasets qualitatively and quantitatively, achieving the state-of-the-art performance in terms of inpainting quality and speed.

==> sections_camera/approach.old.tex <==
\subsection{Stacking Flow Inpainting Network}
Flow inpainting is to fill the area with correct motion of direction and speed. Unlike image inpainting, it is difficult for the model to estimate the missing flow from the single optical flow. However, from the other flows in the video, the model may get much prior information to fill the missing motion like the shape, prior speed and direction. 
The DFI network has been depicted in Figure~\ref{fig:dfi}. Our coarse-to-fine model mainly contains two subnetworks, DFI-C and DFI-S. The DFI-C model to estimate an coarse flow inpainting result in low resolution is made up of ResNet101 and a simple upsampling module containing a convolution layer and upsampling operation. To refine the coarse result, we construct the DFI-S network, composed of ResNet50 and a little more complex upsampling module.
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/DFI_architecture.png}
    \vspace{-16pt}
    \caption{\small{The network architecture of our DFI newwork. \textbf{Best viewed in color.}}}
    \label{fig:dfi}
    \vspace{-15pt}
\end{figure*}
\par{}
\textbf{DFI-C }   As we have mentioned that it's hard for the model to accurately inpaint the flow from the single masked flow, the DFI-C network takes a sequence of 10 consecutive flows with hole and the mask of the each flow as input and inpaint the 6th flow. We can get double directions' flow from any video. Let's denote the ith frame in video as $I_i$, the forward direction flow as $F^{f}_{i}: Flow(I_{i+1}\to I_{i})$ and the reverse direction flow as $F^{r}_{i}: Flow(I_{i-1}\to I_{i})$. During training, we only sample 10 consecutive flows from a single direction. When inpainting videos, we can meet variety of masks among which the size of the mask will be so large that the convolutional neural network cannot handle it. To mitigate this influence on our model, two strategies are employed for coarse the flow inpainting model. Having observed that it's much easier for the model to inpaint the smaller hole, we downsample the input flow by 2 times so that the size of the hole is two times smaller than the original one and the DFI-C network can easily estimate the the flow of the smaller hole in first coarse stage. What's more, we substitute traditional convolution layer with dilation convolution layer to the Resnet101 backbone for much larger receptive field. 
\par{} In the experiments, we find that if we set the hold of the input as 0 just like image inpainting, the training process will be much more unstable. Furthermore, using the simple region fill method to initialize the hole with reasonable value can speed up the training process and this initialization also helps the model to be more robust even if the hole's size is large. 
\par{}
\textbf{DFI-S} Our first stage, DFI-C network, aims to fill the hole of a single flow with coarse result and the DFI-C network seems to have no direct relation with the following flow propagation step. Thereby DFI-S network is to link the flow inpainting to the propagation step and refine the coarse result from DFI-C network in higher resolution. 
\par{}
Motivated by Flownet2, we expect that the deep neural network can benefit from iterative refinement and the input of the refine network can have much more connections with the final propagation step. Given the propagated map and the accumulated errors in the procedure, the model is capable of amending the coarse flow to fit the final propagation. Let's denote $I_i^h$ as the masked ith frame of which the hole will be set to 0, $\hat{F}$ as the coarse flow generated from DFI-C. In the refinement stage, we also sample 10 consecutive flow from a video, but we the first five consecutive flow is from reverse direction and the last five flow is from forward direction. Therefore, the final flow sequence is $[\hat{F}_i^r,...,\hat{F}_{i+4}^r, \hat{F}_{i+4}^f,...,\hat{F}_{i+9}^f]$ and the corresponding masked frame sequence is $[I_{i-1}^h,...,I_{i+9}^h]$. Pay attention that middle two flows have the same index but they are respectively from reverse direction and forward direction. Taking $\hat{F}_{i}^r$ as an example, we can warp $I_{i-1}^h$ by using the single direction flow, $F_{i}^r$. Sequentially, the brightness diff-map $D_{i-1, i}$ is the norm of subtraction of the warped $(i-1)$th frame, $I^w_{i-1}$ and the masked ith frame. The hole of $I_i^h$ may be filled partially by the warped $(i-1)$th frame and we will keep the warped value in $I_i^h$ so that we can iteratively propagate the value to the middle masked frame. For the sake of unity, we use the notation of $\hat{I}_i^r$ to represent the combination of $I_i^h$ and $I_{i-1}^w$ and the superscript 'r' is to indicate the direction of the flow we used. After repeating this operation 5 times, we can get the middle brightness diff-map $D_{i+3, i+4}$ and partially filled frame $\hat{I}^r_{i+4}$ by the 5 consecutive reverse flow sequence. Likewise, it's easier to get another direction's middle diff-map $D_{i+5,i+4}$ and the partially filled frame $\hat{I}^f_{i+4}$ by using the flow sequence $[\hat{F}_{i+8}^f, ..., \hat{F}_{i+4}^f]$ and corresponding frames. The middle color diff-map, $D_{i+4}$, is the subtraction of $\hat{I}^f_{i+4}$ and $\hat{I}^r_{i+4}$. Having construct the 10 brightness diff-map and middle color diff-map, the refinement network take the combination of the brightness diff-map, the middle color diff-map and the middle two coarse flow, $(\hat{F}_{i+4}^r, \hat{F}_{i+4}^f)$, as input and the output is the refinement of $(\hat{F}^r_{i+4}, \hat{F}^f_{i+4})$.

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{figures/diff-map.png}
    \vspace{-16pt}
    \caption{\small{An example of diff-map. \textbf{Best viewed in color.}}}
    \label{fig:diffmap}
    \vspace{-15pt}
\end{figure}

\par{}
In order to have a more intuitive view, we depict the process of generating the diff-map in Figure.Diff-map. According to Figure.Diff-map, we observe that the middle color diff-map has a high degree of coincidence with the difference between the coarse inpainted flow and the ground truth. The brightness diff-map indicate the whole pixel propagating process and each step's bias in the propagation. Given the bias and the propagating process, the model will learn to modify the middle two coarse flow so that the refinement result is able to fit the color propagating process well.  
\par{}
Different from the DFI-C, the DFI-S has a more complex upsampling module which is composed of three-layer convolutional upsampling network alternating convolutions and bilinear two-times upsampling operation and we remove the final non-linear function in this module for the output may not have a fixed range. Note that all of the images have been normed to $[-1, 1]$. 
\par{}
\textbf{Hard Example Mining Loss}  We observe that most area of the flow is smooth and it seems that the common $l_1$ reconstruction loss is compatible with this nature. However, as we only use $l_1$ loss in the hole of the flow to supervise the model, the nature of the flow's smoothness will mislead the model to predict the flow which the edge of separate object's flow is smooth. What's more worse, the smooth edge of flow can cause serious problem in the next propagating step.
\par
The model has worse performance in the boundary as there exists a huge bias in the number of training samples between the sharp region and the smooth region. Intuitively, can we let the model automatically choose the difficult area and add a weight in those areas to enforce the model to learn the sharp feature of flow? Inspired by paper-cite, we sort the per-pixel $l_1$ loss and set a threshold $th_{hard}$. All of the pixels whose $l_1$ loss is bigger than $th_{hard}$ will be labeled as hard samples. Then, those pixels' $l_1$ loss will be multiplied by a weight denoted as $\lambda_{hard}$ to enforce the model to pay much more attention to the sharp features of optical flow.

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{figures/hard-example-mining.png}
    \vspace{-16pt}
    \caption{\small{An example of the result of hard example mining. \textbf{Best viewed in color.}}}
    \label{fig:hard}
    \vspace{-15pt}
\end{figure}

\par
As depicted in Figure.HEM, we add this hard example mining loss in DFI-S network in the settings of the hole is a square in the mid of the the video. In the second column of this figure, the hard examples' area has been labeled as white. As we can see from that, the hard examples mainly distributed around the high frequency area like boundaries. Having a further comparison between the coarse result in third column and the refinement result in the final column, we can easily observed that the model grasps the ability to handle the sharp features in optical flow.
\subsection{Flow Guided Color Inpainting}
\par
\textbf{Flow Guided Color Propagation} Generated by DFI network, the inpainted optical flow can construct the chain of each pixel in the frame's pool. By the definition of the optical flow, we can use the simple warping operation to propagate the color from the last frame to the current frame, so in the temporal-spatial space the chain can fill the masked region with some unmasked pixels.
\par
As we have the optical flow of forward direction and backward direction, we will propagate the color in each direction so that we can take the most advantage of the unmasked pixels. Taking the reverse direction's flow as an example, we show the detailed propagation procedure in Algorithmn\ref{algo:algo}. Let's denote $\tilde{F}$ as the final refined optical flow, the mask of the ith frame in which the hole is set to 1 and the rest to be 0 as $M_i$. Likewise, the other direction's propagation is similar to Algorithm.\ref{algo:algo}. After the double direction's propagation, $results_r$ and $results_f$ store the intermediate results of each frame in the video and the $time\_stamp$ stores the index of the frame where the hole's pixels come.In the end, according to the distance between the current frame index to the each time stamp, we average the $results_r$ and $results_f$ to get the final result sequence.

\begin{algorithm}[ht]
\caption{Flow Guided Color Propagation by using reverse direction's flow}
    \begin{algorithmic}[1]
    	\State{Initialize $results_r[i] = I_{i}^h$, $time\_stamp_r[0][M_0==0]=0$ and set $th=10$}
    	\For {\(i = 1, ..., frames\_num\)}
			\State{Get $\tilde{F}_{i-1}^f$, $\tilde{F}_{i}^r$, $M_i$}
			\State{Initial $results_r[i]=I_i^h$, $time\_stamp_r[i][M_i==0]=i$}
			\State{Get warped flow $\tilde{F}_{i-1}^{warped}$ by using $\tilde{F}_i^r$ to warp $\tilde{F}_{i-1}^f $}
			\State{Get the valid flow map $V$: norm($\tilde{F}_{i-1}^{warped} - \tilde{F}_i^r$) $< th$}
			\State{Update the hole of $results_r[i]$ by using $\tilde{F}_i^r$ to warp $results_r[i-1]$. According to V, the invalid region won't be updated}
			\State{Update $time\_stamp_r$ like $results_r$}
		\EndFor
    \end{algorithmic}
\label{algo:algo}
\end{algorithm}
As the estimated flow may be inaccurate in some points, we check the validity of the flow by the valid flow map $V$ in Algorithm.\ref{algo:algo}. If the pixel is filled by the invalid flow, we won't update the pixel in the hole and the chain won't connect the unmasked pixels to masked region.
\par
\textbf{Inpaint Unseen Regions in Video}
In some case, some region cannot be filled by the unmasked pixels in the pool of the whole frames, which means that the model cannot connect the certain masked regions to any unmasked pixel. Therefore, inpainting the left region is just a problem of image inpainting. Following the work of Deepfillv1 paper-cite, we construct our image inpainting model. Among the sequence to be inpainted , there may exist more than one subsequence we cannot inpaint by color propagation. We just use the image inpainting model to fill the first and the last frame in each subsequence and then the color will be propagated again by the inpainted flow. As we have already used the color propagation to inpaint the majority of the masked region, the left hole can be easily inpainted by the image inpainting model.












